Impact of Geo-distribution and Mining Pools on Blockchains: A Study of Ethereum

Given the large adoption and economical impact of permissionless blockchains, the complexity of the underlying systems and the adversarial environment in which they operate, it is fundamental to properly study and understand the emergent behavior and properties of these systems. We describe our experience on a detailed, one-month study of the Ethereum network from several geographically dispersed observation points. We leverage multiple geographic vantage points to assess the key pillars of Ethereum, namely geographical dispersion, network efficiency, blockchain efficiency and security, and the impact of mining pools. Among other new findings, we identify previously undocumented forms of selfish behavior and show that the prevalence of powerful mining pools exacerbates the geographical impact on block propagation delays. Furthermore, we provide a set of open measurement and processing tools, as well as the data set of the collected measurements, in order to promote further research on understanding permissionless blockchains.

==> background.tex <==

%%%%%%%%%%%   BACKGROUND   %%%%%%%%%%%
\section{Background}
\label{bg}

In this section, we provide some background on blockchains in general and Ethereum in particular.
We focus on the general high-level aspects rather than the low-level protocol details and formats.
For the latter, the interested reader can refer to the Ethereum's yellow paper~\cite{Ethereum} and the official Ethereum documentation~\cite{etherdocs}.
%In this section we give a brief introduction to Ethereum, adding the details that will be needed later in this paper.
Ethereum is a permissionless blockchain that provides a platform for developing and implementing decentralized applications --- known as Smart Contracts.
Ethereum also acts as a cryptocurrency by providing its own currency, known as Ether. 
Both the state of the currency and of the Smart Contracts is maintained in the blockchain, a public append-only ledger that keeps track of all state changes. 
The state of the system is associated with accounts, which are stateful objects whose states --- e.g. account balance or Smart Contract variable --- can be changed through transactions.
There are two types of accounts: externally owned ones which are controlled by user's private keys and contract accounts associated to Smart Contract code. %represented by a code controlled by messages.

The system runs on a peer-to-peer network basically consisting of three types of peers:
\begin{description}
  \item [Bootstrap nodes:] Highly-available peers run by volunteers whose purpose is to facilitate the connection of new clients.
  \item [Miners:] Peers who produce --- i.e. \emph{mine} ---  new blocks and spread them across the network.
  \item [End users:] Common participants of the platform that send and receive transactions, deploy smart contracts, etc.
\end{description}


In the rest of the section, we provide an overview of the main concepts underlying Ethereum.


\subsection{Transactions}
Transactions are the main mechanism to update the state of the system.
All transactions are signed by the account that submitted them to the system.
%refers to the signed data package assembled by externally owned accounts.
Transactions have two different uses: i) to indicate a simple currency transfer between accounts or, ii) to deploy or invoke operations in Smart Contracts.
%They are later propagated to the network as described in Section~\ref{tx-lifecycle}. 	
A transaction contains several fields, of which the most important are: the address (public key) of the recipient, the value of Ether to be sent, the Smart Contract code, and the \emph{nonce} indicating the total number of transactions sent from the account, and used to ensure the transactions emitted from an account are executed in the desired order.

To prevent flooding the platform with useless or spurious transactions, as well as to forbid the execution of Smart Contracts with infinite loops, Ethereum implements an internal pricing system in the form of gas. 
Each transaction's code -- be it a simple value transfer or a contract call -- is a collection of opcodes, where each opcode costs a pre-determined amount of gas. 
The creator of the transaction cannot modify this cost, but she is free to choose the \emph{gas price} --- the amount of Ether she is willing to pay per one unit of gas to the miner for including such transaction in a block. The transaction fee then equates to the product of the amount of gas spent and gas price per unit.


\subsubsection{Transaction lifecycle}
\label{tx-lifecycle}

Transactions are disseminated over the network using an epidemic, or gossip-based, protocol.
Briefly, when a user creates a new transaction, she broadcasts it to all the neighboring peers.
Upon a transaction reception, the nodes forward the transaction to their neighbors -- usually just to a limited number of them -- which in turn will forward it to their neighbors.
Eventually, the transaction will reach a miner node.
Miners perform a process called \emph{mining} -- described in more detail in \S\ref{subsec:mining} -- which leads to the insertion of the transaction into a new block. 
Miners then propagate the block back to the network also following a gossip style protocol.
Peers eventually receive the block, verify its validity, and update accordingly their local copy of the blockchain.

It is important to note that the information propagation strategies and the client behavior in general are not standardized in Ethereum. 
For instance, the Geth client (v1.8.23) maintains connections with 25 other nodes, whereas Parity connects to 50 peers.
Currently, there are 8 different client implementations written in different languages, all following the WIRE\footnote{https://github.com/ethereum/devp2p/blob/master/caps/eth.md} protocol specification, but their logic substantially differs from each other.
This heterogeneity implies that it is challenging to accurately infer the behavior of the network by carefully studying all implementations, and rather one needs to resort to observing and measuring such behavior in the real deployment over a long time period.


\subsection{Blockchain forks}
The Ethereum protocol aims for a block interval -- the mean time it takes to mine a new block -- between ten to twenty seconds. 
This is ensured by continuously and automatically adjusting the mining difficulty.
On one hand, the low block interval -- $\sim$40 times shorter than in Bitcoin --  allows for better response time, which is a desired property in cryptocurrencies, and for better throughput.
 On the other hand, short block intervals lead to an increased amount of forks, i.e. events where two competing miners produce two blocks that reference the same preceding block.


%Huge forked block rates in classical Nakamoto's consensus impede less powerful miners, as they are less likely to mine a block fast enough, thus leading to mining centralization. They also weaken the absolute strength of the network against attacks, as the inventor and co-creator of Ethereum Vitalik Buterin explains in his blog post\footnote{https://blog.ethereum.org/2014/07/11/toward-a-12-second-block-time/}.
%Ethereum, as a countermeasure against the unpleasant consequences of the short block interval, implements a modified version of the Greedy Heaviest Observed Subtree (GHOST) protocol~\cite{GHOST}.
Given a fork, miners have to decide which path to consider as valid.
The original Nakamoto's consensus protocol~\cite{Bitcoin} considers the longest chain as the one which represents the current state of a blockchain network.
This implies that blocks that are not included in the main chain are discarded, together with the mining effort spent to produce such blocks.
Ethereum adopts another strategy by relying on a modified version of the Greedy Heaviest Observed Subtree (GHOST) protocol~\cite{GHOST}.
The intuition is simple, rather than completely discarding blocks that did not end up in the main chain, Ethereum allows blocks in the main chain to reference blocks outside the main chain --- known as uncle blocks.
Therefore, the weight of a chain is calculated from the cumulative difficulty of the main chain and uncles. 
The Ethereum GHOST modification deviates from the original one in the fact that it rewards not just the blocks on the main chain, but the uncles as well. 
The goal is to incentivize small miners, and hence mining decentralization, by promoting a fairer distribution of rewards among miners.
Moreover, this also strengthens the security of the blockchain as a malicious actor needs to construct a chain that is \emph{heavier} than the main chain plus the corresponding uncle blocks.
Finally, blocks that are not included in the main chain nor referenced by any blocks are called unrecognized forks and do not contribute to the security of the blockchain.


Note that despite the fact that Ethereum distributes rewards to uncle blocks, only transactions included in main blocks affect the state of the system and transactions in the uncle blocks are ignored.
When coupled with the occurrence of forks, this implies that when a node observes a new block B, it is not safe to immediately consider the state transition given by the transactions in block B, because there is a chance that B might be considered an uncle or unrecognized block at a later point in time.
Therefore, nodes must wait for a \emph{long enough} suffix of blocks to ensure that the appearance of an alternative heavier chain, where block B is not included, has a small probability. 
This property is known as block finality.
In Ethereum, nodes wait for a suffix of 12 blocks before considering a block final --- and thus consider the transactions that affect the blockchain state valid~\cite{blockConfirmation}.
Note, however, that due to the nature of Proof-of-Work (PoW), block finality is always probabilistic as there is always a non-zero chance that an alternative heavier chain appears.


Our observations, discussed in more detail in \S\ref{Analysis}, provide some surprising results on the topics we just discussed.
On the one hand, the rewards of uncle blocks, which are supposed to incentivize a fairer share of rewards, are in fact being exploited by mining pools to further increase their gains.
On the other hand, we observed that mining pools have been able to mine large continuous sequence of blocks putting into question the rule of thumb of the 12 confirmation blocks.


\subsection{Mining process}
\label{subsec:mining}
The role of miners is to validate transactions and orderly collect them in blocks.
Mining rewards a successful miner with a fixed amount of Ether coins per block, along with transaction fees for every transaction included in the newly mined block.

\subsubsection{Proof-of-work}
Miners, in addition to validating transactions, must perform a technique called Proof-of-Work (PoW) which consists of resolving a computationally expensive cryptopuzzles.
Under the hood, PoW consists of repetitive hashing of a string consisting of the block's data and a nonce.
The goal is to find a nonce such that the resulting hash is less than a certain threshold -- determined by the difficulty of the network. 
Because the hash function is assumed to be practically non-invertible, the only way to solve the puzzle is through brute force.
After finding a solution, the block is valid and can be propagated to the network.
%A miner tries to perform the computations for a tremendous number of nonces until the final produced hash 
% TODO     - more reasons for pOw -> ( preventing Sybil attacks ?? )
The fact that PoW is very hard to perform guarantees the security of the platform since it makes it resistant to being flooded by false blocks and makes potential future modifications of previously confirmed parts of the blockchain almost impossible. Furthermore, it makes miners spend some time performing the computations, allowing the rest of the network to have enough time to synchronize.
Due to the computational complexity of mining in the Ethereum network, it is practically impossible for an individual running a personal computer to find new blocks. For this reason, mining is performed either in powerful clusters or, even more often, in mining pools. The latter are discussed in \S\ref{subsection:miningpools}.

Finally, PoW is not the only possible consensus algorithm and the Ethereum developers are intensively researching other options, e.g. Proof-of-Stake, which this paper will not cover. The main reason for switching to another strategy is the environmental threat the PoW causes due to the enormous amount of electricity\footnote{https://digiconomist.net/ethereum-energy-consumption} consumed by the mining instances.


%\subsection{Information propagation}
%\label{subsection:infoPropag}

%The efficiency of the Ethereum platform largely depends on the time it takes for transactions to propagate from users to miners and the time it takes for a transaction to get committed \cite{**}.\jpb{we need to define commit.} \jpb{can't we state the same thing about block propagation time?}

%In general, the transaction flow is the following:
%when any Ethereum participant decides to create a new transaction, it broadcasts it to all neighboring peers they are connected to. \jpb{you should have said that peers are connected to K neighbors, and summarize how those connections are set up.}

%A miner includes the transaction into a new block only if: its parameters are valid, the funds are sufficient, the signatures match and if the miner finds the offered fee to be profitable for them. \jpb{you haven't said anything about funds, signatures and mining fees before. you should, otherwise this sentence will not be clear.}

%Finally, miners propagate the transaction back to the network inside a newly mined block. %The Ethereum protocol supports direct whole block messages as well as light new-block announcements that
%After receiving the new block, each peer verifies whether the block's nonce leads into some specific mixHash. Then they verify and execute the individual transactions and synchronize so with the Ethereum platform.\jpb{need to define nonce, mixHash.}


\subsection{Mining Pools}
\label{subsection:miningpools}

The increasing popularity and market capitalization of Ethereum over the years led to a increase in the number of miners.
While this is generally good, as more miners make the network more secure and harder to attack, it also means that the mining difficulty needs to increase proportionally to the mining power in the network.
The downside of this increase in mining difficulty is that regular miners, who use commodity hardware at home, have more difficulty in successfully mining a block and collecting the respective rewards.
Mining pools address this problem by congregating the mining power of multiple users into a single entity.
A typical mining pool consists of a private network running a control server that splits and distributes the workload among individual miners. The workload consists of a Merkle root of a set of transactions and a range of nonces to search through.
The individual participants of mining pools skip the validation phase and solve just a \emph{subpuzzle} of the full cryptographic puzzle, with a lower difficulty.
When a participating miner finds a solution for the puzzle, he sends it to the server, which uses that information to generate the final block and propagates it to the Ethereum network.
The miners are later rewarded in proportion to the computational resources they spent. %The pool typically charges a fee of around one percent\footnote{https://www.cryptocompare.com/mining/\#/pools}.


Currently, there are growing concerns about the power of mining pools on the Ethereum network.
As a matter of fact, just four mining pools control $\approx 70\%$ of Ethereum's total mining capacity which poses some threats to the network security as we will discuss below~\cite{ethPool}. 
Moreover, in our study, we also found evidence that mining pools have been able to mine a large sequence of consecutive blocks which raises concerns about the wisdom of waiting just for 12 confirmation blocks before considering a block as final.

\subsection{Security}

%\subsubsection{Platform security}

% no 50%-miner assumption
The security of the Ethereum platform depends on the assumption that no miner, mining pool, or colluded set of miners, is more powerful than the rest of the network, as that would enable that miner to replace recent blocks and perform double-spending of funds, among other attacks.
It is believed that this assumption is realistic as long as: i) miners are rational, i.e., it is more profitable for them to follow the protocol than to attack it, and ii) miners do not join pools that are too powerful~\cite{Luu2017}.
The intuition is that if miners did that it would make a successful attack trivial (for instance if all miners joined the same pool, that pool could censor transactions and rewrite the blockchain), thus hindering the trust in the platform and making the value of the Ether currency decline.


From the perspective of the end users, and assuming that miners remain rational, the main concern is the issue with block finality discussed above.
It is important to mention that transactions may never commit. 
First, miners can  refuse, for any reason, to include a transaction in a block. Second, even after getting included in a block, that block may not become part of the main blockchain. One can be sure that a transaction will never commit when another transaction from the same account with the same nonce gets committed.
We will discuss these behaviors, among other in \S\ref{Analysis}. 

%\subsubsection{Commit of transactions}
%The existence of forks and the uncertainty about which block will eventually become the part of the main blockchain leads to the need to wait for 12 confirmation blocks to consider a transaction committed.
%The creators of Ethereum argue that this number of blocks~\footnote{https://ethereum.stackexchange.com/questions/183/how-should-i-handle-blockchain-forks-in-my-dapp/203\#203} is sufficient to guarantee the near impossibility to replace such blocks.
%
%







% SKIP   AS   IT   DOES   NOT   RELATE  WITH OUR PAPER
%\subsubsection{End user security}
%The security of funds allocated on Ethereum accounts rely on elliptic curve cryptography which is generally perceived as unbreakable\footnote{TODO Add citation - NSA ref doc} on contemporary computers.
%Therefore, as long as the end users keep their private keys protected, they should not have to worry about an attack breaking the cryptography.



==> cat-future-work-plan.tex <==
\section{Ongoing PhD work}
\newcommand{\docname}{work}
\newcommand{\name}{novel algorithm}
\newcommand{\model}{hybrid consistency}
\newcommand{\nameendAGTattack}{forced fork attack}
\newcommand{\listA}{\emph{maybe-admitted}}
\newcommand{\listB}{\emph{inadmissible}}

\label{sec:concludedwork}
%\subsection{Hybrid consistency model}
The strongly consistent, yet high-latency, commit guarantees of PoW consensus
are inappropriate for many geo-distributed applications.
Further, our experiment suggests this high latency is increasing, as
applications are expected to need to wait for more confirmation blocks for security.
To mitigate this problem, our ongoing work focuses on 
a novel algorithm that extends blockchains 
with an additional weakly-consistent view of the replicated ledger.
This view has a significantly lower latency than current commit
views of existing blockchain systems, while offering a censorship-free 
and causally-correct ledger.
%, which handles conflicts consistently. 
%For many geo-distributed applications, 
The weakly-consistent ledger is a fast path to support those operations of an 
application that do
not require strong consistency.
We are designing it as a pluggable extension
to existing blockchains such as Bitcoin and Ethereum.
\iffalse % begin comment out
\subsection{Improved gossip-based transaction dissemination}
\label{sec:cat:probbcast}
In the first stage of developing our novel algorithm, 
we assumed the existing Ethereum transaction dissemination
protocol is able to reach all nodes in the system within a bounded time
with high probability. However, %this protocol suffers in practice from several deficiencies, 
%such as %high latency for a number of nodes ~\cite{Sirer2018} and 
transactions may not reach
every node when broadcast~\cite{OnAvailability--01}, which may 
compromise this assumption. 
To overcome this problem, we intend to improve the existing Ethereum
probabilistic gossip-based dissemination protocol. %, in \S~\ref{sec:alg:attacks}. 
%Upon inspection of the existing Ethereum transaction dissemination
%protocol implementation in Geth, we observed it uses a variant of \textit{eager push}~\cite{leitao2010gossip}, where nodes send the full
%transaction payload to all their neighbors (as opposed to the standard eager push, 
%where a random subset of known nodes is selected), 
%and on the \textit{infect and die} model~\cite{eugster2004epidemic}, where nodes
%disseminate a transaction upon seeing it for the first time, but take no further action when
%receiving duplicates.	
%We will implement changes to the existing protocol, incorporating concepts from
%previous work like EpTO (Epidemic Total Order)~\cite{Matos2015}
%and including parameters such as peer fanout, number of times an event needs to be relayed and time
%between event relay rounds, which can be adjusted to the characteristics of a given deployment. 
%As a consequence, nodes may be required to connect to more neighbors to increase peer fanout 
%and an increased number of dissemination messages being sent to the network is anticipated
%(due to flooding from eager push, for generating message redundancy~\cite{leitao2010gossip}), 
%after adjusting the relevant parameters. We expect this to allow us to fulfill the goal of reaching all nodes 
%within AGT with high probability, by decreasing transaction dissemination latency and transaction loss.
%Further, Leit{\~a}o \textit{et. al}~\cite{leitao2010gossip} stated that using TCP in a gossip protocol allows using 
%more conservative values for fanout than traditional UDP systems. 
%Ethereum already uses TCP in its gossip protocol and we will also keep using it due to its lower fanout.
%Frey \textit{et. al}~\cite{frey2010boosting} described how Byzantine nodes can attack gossip: i) attack the peer sampling; ii) pollute the protocol %to decrease performance and 
%to increase load on all nodes and lead to a DoS. We will attempt to make our protocol resilient to such attacks.
% paulo: fica a faltar talvez dizer que os trabalhos anteriores eram para ambientes do tipo crash e que o nosso e' bizantino
%We expect this implementation to be pluggable to other blockchain platforms.

%After the implementation, we will measure the network usage impact of the resulting algorithm. 
% weaker reliability of the transaction delivery protocol
%We will also evaluate how \name will behave in scenarios in which the intended probabilistic guarantees are not possible,
%or are too costly.
%To that end, we will run experiments with more challenging network conditions such as
%very high latency (i.e., transaction delay resulting in transactions being placed in the \listA and \listB lists
%or being discarded) and message loss (i. e., transactions and blocks not delivered to all nodes).
\fi % end comment out
%\subsection{Adding hybrid consistency to smart contracts}

%An important fraction of applications that can benefit from our novel algorithm are
%developed by interacting with Ethereum smart contracts. 
We plan to study the integration of our hybrid 
consistency model into smart contract languages like EVM assembly or Solidity \cite{Luu2017}.
%Currently, when externally invoking a method for querying a smart contract
%value (that is, a method that returns a value but does not change any
%internal variables), the returned value reflects the last executed transaction
%that changed the smart contract state. We can consider this transaction
%as \textit{committed}, if it is present in a block that already had $C$ subsequent
%blocks produced after it, or as \textit{uncommitted} otherwise. This is a problem
%for such applications, since they are not aware of the consistency
%guarantees that are offered for the returned value and may be relying on an
%uncommitted value.
We intend to fill this gap by explicitly allowing applications to request a
desired consistency level for the returned value, when invoking such smart
contract methods. 

%Namely, applications will be able to request the 
%following consistency levels:
%\begin{enumerate}
%	\item \textit{Legacy}: Provides the same value as Ethereum today, that is, the
%	value corresponding to the last transaction in a block that changed the corresponding
%	smart contract state.
%	\item \textit{Admitted}: Provides the value resulting from the last admitted transaction that changed
%	the corresponding smart contract state, respecting \model. 
%	This transaction may not have yet been included in a block and it may be ephemerally executed 
%	(i.e., executed to a temporary memory space without becoming permanent).    
%	\item \textit{Committed}: Provides the value resulting from the last committed transaction
%	that changed the corresponding smart contract state. More recent transactions changing this state
%	may already have been executed, but the returned state must not reflect them. It should
%	reflect transactions with $C$ blocks after them.
%\end{enumerate}

%To provide these consistency levels, we anticipate a new layer between
%the smart contract external invocation and the global Ethereum smart contract state.

%For the \textit{Admitted} consistency level, whenever a smart contract method for querying a value is
%invoked requesting this consistency level, we will retrieve all the admitted transactions
%that have not been executed and will execute them in the Ethereum Virtual Machine~\cite{Evm2018}. The
%resulting state will be stored in a temporary memory space instead of becoming permanent and 
%will be used when executing the invoked method.

%For the \textit{Committed} consistency level, we will also store the previous global state that would result 
%from not having executed the last $C$ blocks.  Thus, whenever a smart contract method that queries a value is
%invoked requesting this consistency level, this previous global state will be used.


%\subsection{Weaker probabilistic assumptions}

%We plan to study, both formally and empirically, what is the impact 
%that weaker probabilistic assumptions (namely, the  
%reliability of the transaction delivery protocol and the guarantees of PoW commit)
%effectively have on probabilistic guarantees provided by \name.

%% weaker reliability of the transaction delivery protocol
%In \S~\ref{sec:cat:probbcast}, we proposed improving the blockchain dissemination components
%with more reliable probabilistic guarantees. Nonetheless, it is important to assess how
%\name will behave in scenarios in which such probabilistic guarantees are not possible.
%We will thus try to run experiments with more challenging network conditions such as
%very high latency (i.e., transaction delay resulting in transactions being placed in the \listA and \listB lists
%or being discarded) and message loss (i. e., transactions and blocks not delivered to all nodes).

%% weaker guarantees of PoW commit
%We have previously considered a transaction $t$ as \textit{committed} after $C$ blocks have been 
%produced after a block including $t$, using PoW. 
%However, this is a probabilistic assumption, which means that theoretically
%a malicious user could produce a chain that is slightly longer than $C$ (with very low probability). 
%We will try to assess how \name behaves when the PoW guarantees are not met (i.e. when more than $C$
%blocks are replaced).

%Previous work has set a theoretical limit on the minimum block time without risking security and related it with the
%block transmission time \cite{Kiayias2015speed}. We will try to assess the effect of reducing block size in \name,
%when attempting to minimize the block time and consequently improve the commit time.

%\subsection{\model with no PoW}

%Another direction is to study how the \model could be used without requiring PoW.
%We will evaluate whether \name could be used with blockchains using emerging 
%alternatives to PoW, such as Byzantine Agreement (BA) protocols, Proof-of-Stake (PoS) \cite{Berger2018} and Proof-of-Space (PoSp) \cite{Kiayias2017}.
%The \textit{committed} guarantee will have to be provided using the corresponding guarantees
%in those technologies.  As an example, the Algorand blockchain has been described as confirming transactions on the
%order of a minute, with a negligible fork probability \cite{Gilad2017}. Using \name with Algorand can thus mean having even lower commit times
%than with Ethereum on average, in case forks are as negligible as described, and having the \model model available.



%Table \ref{tab:wkplan} presents our workplan.

% https://www.tablesgenerator.com/
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
%\begin{table}[!hbt]
%\begin{tabular}{@{}llllllllllll@{}}
%\toprule
%Activity                & 2019                     &                                                 &                          &                          &                                                 &                                                 &                                                 &                                                 & 2020                                            &                                                 &                                                 \\ \midrule
%Probabilistic broadcast & \cellcolor[HTML]{FE996B} & \cellcolor[HTML]{FE996B}                        &                          &                          &                                                 &                                                 &                                                 &                                                 &                                                 &                                                 &                                                 \\
%Smart contracts         &                          & \cellcolor[HTML]{FE996B}{\color[HTML]{F8A102} } & \cellcolor[HTML]{FE996B} & \cellcolor[HTML]{FE996B} & \cellcolor[HTML]{FE996B}                        &                                                 &                                                 &                                                 &                                                 &                                                 &                                                 \\
%Weaker assumption       &                          &                                                 & \cellcolor[HTML]{FFFFFF} & \cellcolor[HTML]{FE996B} & \cellcolor[HTML]{FE996B}{\color[HTML]{FE996B} } & \cellcolor[HTML]{FE996B}{\color[HTML]{FE996B} } & \cellcolor[HTML]{FE996B}{\color[HTML]{FE996B} } &                                                 &                                                 &                                                 &                                                 \\
%No PoW                  &                          &                                                 &                          &                          &                                                 & \cellcolor[HTML]{FE996B}{\color[HTML]{FE996B} } & \cellcolor[HTML]{FE996B}{\color[HTML]{FE996B} } & \cellcolor[HTML]{FE996B}{\color[HTML]{FE996B} } &                                                 &                                                 &                                                 \\
%Thesis writing          &                          &                                                 &                          &                          &                                                 &                                                 & \cellcolor[HTML]{009901}{\color[HTML]{009901} } & \cellcolor[HTML]{009901}{\color[HTML]{009901} } & \cellcolor[HTML]{009901}{\color[HTML]{009901} } & \cellcolor[HTML]{009901}{\color[HTML]{009901} } & \cellcolor[HTML]{FFFFFF}{\color[HTML]{009901} } \\ \bottomrule
%\end{tabular}
%\vskip 5mm 
%\caption{Work plan}
%\label{tab:wkplan}
%\end{table}



==> intro-docforum.tex <==
%%%%%%%%%%%   INTRODUCTION   %%%%%%%%%%%

\section{Introduction}

%trabalhos anteriores focaram-se num conjunto incompleto de metricas (ou seja, nao cobrindo todos os pilares fundamentais da tecnologia) e na perspetiva de um observador apenas (ou seja, sem visao 'a escala planetaria)

Over the recent years, permissionless blockchains have enjoyed rapid growth and gathered remarkable interest. % -- no longer just from technological enthusiasts, but from the general public as well.
 Permissionless blockchains enable cryptocurrencies and other distributed applications based on smart contracts that promise to
 revolutionize the current payment methods with the
 ambition to eliminate the need for banks or other centralized entities acting as trusted mediators of financial operations. 
% The goal of the technology is to guarantee an honest and proper execution of user transactions that can be verified by anyone that joins the system.
% Furthermore, permissionless blockchains can also support Smart Contracts, which introduce a game-changing paradigm for building new kinds of byzantine fault-tolerant geo-distributed applications~\cite{Yellow,SmarterContracts,ConcurrentPerspective}. 
% These appealing features led to a wide adoption by users resulting in a market capitalization in the order of the thousands of billions of dollars~\cite{marketCap}.

At the core of most permissionless blockchains lies a conceptually simple protocol, such as the Proof-of-Work (PoW) consensus proposed by
Nakamoto~\cite{BitcoinShortened}, which specifies the rules on how the blockchain % underlying replicated ledger 
should grow and converge.
%how the replicated ledger grows and converges consistently.
Despite this simple core mechanism, real-world permissionless blockchain deployments 
such as Bitcoin~\cite{BitcoinShortened} or Ethereum~\cite{Yellow},
are extremely complex systems composed of several modules and protocols whose properties are intrinsically hard to understand.
%To further complicate matters, not all implementations follow the specifications, while different clients have
%different default parameters \cite{Parity2019, Geth17DefaultConfig}. 

%%\jpb{We should revise this list of ``real-world issues'', I just wrote it from scratch, so I may well be missing important points.}
%As a matter of fact, permissionless blockchains protocols coordinate a vast and
%geographically-distributed system of nodes by resorting to epidemic protocols
%whose emerging behavior is inherently probabilistic and hard to model.
%The set of nodes is open by nature, which provides users with a
%considerable margin to behave selfishly or maliciously.
%This adversarial environment is a further obstacle to any attempt to accurately
%understand and predict the emerging characteristics of the system.
Additionally, permissionless blockchains have long evolved from a plain organization composed of individual miners, to an ecosystem dominated by mining pools. % that reorganize the mining resources in complex and opaque ways.
At the time of writing, the top four mining pools have around 60\% and 70\% of Bitcoin's and Ethereum's total network capacity --- the top permissionless blockchains ---
respectively~\cite{btcPoolNoAccess,ethPoolNoAccess}.
Finally, they rely on a large code-base that includes different implementations (and versions) of the software that blockchain nodes and clients run.
It is fundamental to see how they behave, what doesn't work and opportunities for improvement. 

%Given the large adoption and economical impact of blockchains --- which is expected only to grow in the next decade~\cite{gatnerVal} ---, the complexity of the underlying systems, and the adversarial environment in which they operate, it is therefore fundamental to properly study and understand the emergent behavior and properties of these systems. 
Recent work has performed measurement studies of popular
permissionless blockchains~\cite{InfPropagaion--02, OnAvailability--01,
MeasEthPeersShortened, Sirer2018}. Together, these studies have contributed
to a better understanding of how these intricate large-scale systems perform in practice, 
unveiling some findings that were not originally anticipated.
Still, the general picture attained by these studies is inaccurate and incomplete. This is mostly due to some key limitations: 
%(i) previous studies either focus on one or few facets of the whole system~\cite{InfPropagaion--02, OnAvailability--01, MeasEthPeers, Sirer2018}, instead of following a holistic analysis that considers the remaining fundamental facets;
(i) relying on a single observation point, therefore neglecting how the geographical distribution of the network affects such measurements~\cite{InfPropagaion--02, OnAvailability--01};
(ii) not considering the recent predominance of mining pools as first-class components in today's blockchain landscape~\cite{InfPropagaion--02, OnAvailability--01,
MeasEthPeersShortened};
(iii) ignoring transaction commit time and how it can be negatively impacted by network delays, out-of-order transactions and empty blocks
\cite{Sirer2018,MeasEthPeersShortened}.

We start by describing our experience and lessons
learned on implementing and deploying a measurement infrastructure across different
continents, addressing some of the limitations of previous studies.
We focus on the Ethereum blockchain, the second most valuable cryptocurrency. % and the leading decentralized platform for Smart Contracts.
An extended description of our study can be found in \cite{Silva2020}.
%To achieve this, 
We implemented and deployed a measurement infrastructure
consisting of several especially modified Ethereum nodes placed across different
continents.
Our measurement nodes run an instrumented variant of the Geth open-source
implementation of Ethereum clients. Each measurement node can connect to the main network and collect the desired measurements from the transactions and blocks it observes.
We analyzed long-running measurements acquired by four measurement nodes which were
deployed in North America (NA), Eastern Asia (EA), Western Europe (WE) and Central Europe (CE). 

% We use it to perform a long-lasting measurement with the goal of collecting
% and analyzing a wide range of network metrics, as well as examining several
% until now never studied blockchain properties.


We highlight the following key results of our study:
i) We identify the generalized and consistent practice of different forms of selfish behavior that harm the throughput of the main blockchain. To the best of our knowledge, these practices were not documented and/or not empirically studied systematically
before;
ii) We confirm that the geographical location has a relevant impact on block reception times and that the prevalence of powerful mining pools exacerbates such
effect; 
iii) We provide empirical evidence that the standard 12-block confirmation
rule of Ethereum may not provide the strong probabilistic
guarantees on block finality that are usually assumed in literature;
%\item We confirm prior findings that were considered as part of our metrics, now with updated trends.
iv) We confirm that some of the metrics collected by previous works still present the same values and report relevant changes to other such metrics.

% Our study confirms some previously documented findings but from a multi-observer approach.
% Most importantly, our study sheds new light on the characteristics of Ethereum, as of today, with some additional new findings.
% Among others, we highlight the following:


% \begin{itemize}

%   % joao: the following items need to be revised
  
% \item %geo position influence
% To the best of our knowledge, we are the first ones to measure the block propagation delays and to identify that peers placed geographically closer to mining pools synchronize faster.

% \item % min. pools create forks (blocks with the same height) ..
% We find that prominent mining pools exploit the uncle block reward system and intentionally mine outdated blocks.

% \item % censorship
% Finally, we observe that blockchain consists of long sequences of blocks mined by a unique entity, which enables the possibility of transaction censorship. In consequence, we argue that the current rule of thumb of 12-confirmation-blocks waiting time is not sufficient.

% \end{itemize}



% Previous work~\cite{OnAvailability--01} from 2017 studied various  properties
% of the Ethereum platform, such as what impact the user-defined variables
% "gas price" and "gas limit" have on transaction inclusion, the commit time
% of transactions or the ratio of blockchain forks.
% We replicate and verify their measurements in order to observe how the
% properties changed over the last two years.
% Moreover, we take attention at details, that the authors of ~\cite{OnAvailability--01} omitted, such as the relation between fork lengths and the probability of being referenced in main blocks.
% On top of that, we measure various metrics regarding the forked blocks, e.g. the degree of transaction reordering, and add several other metrics, such as the degree of redundant receptions of new block announcements, with the aim to observe the network traffic overhead.

% Although Ethereum has been out and running for several years and a growing body of research has thoroughly studied it, we were missing an analysis of the Ethereum's underlying network concerning the inconsistencies amidst individual nodes and measuring the propagation delays of information.

% In this work, we are interested in measuring and evaluating the network characteristics of the currently second most valuable cryptocurrency, Ethereum.
% Ethereum opearates on an underlying peer-to-peer network protocol which must support the interconnection of a large number of peers spread all over the world, prevent the creation of network partitions, and allow for a smooth transfer of all the data needed in the system.
Our main contributions are the following:
i) A one-month study of the Ethereum network from several geographically dispersed observation
points;
ii) A set of open-source measurement and processing tools that allows other researchers to reproduce our observations and/or perform similar studies in other blockchain
systems;
iii) The collected data set which might enable other researchers to do other findings in our collected data or refine our
observations. %\footnote{For double-blind purposes both the code and the data set is currently withheld. We will make both publicly available to the community.}

%Briefly, we rely on a multi-observer approach in which our measurements were obtained at multiple geographically-dispersed observer nodes.
%This allows us to 
%We assess the impact of the geographic location in key metrics. 
%For instance, we show that block propagation time is highly skewed, allowing peers in some regions to observe first a large portion of the total blocks --- which gives them a competitive advantage when mining.
%We leverage these multiple observation points to assess the key pillars of Ethereum, namely network efficiency (\S\ref{subsec:netEff}), geographical dispersion (\S\ref{subsec:geoImpact}), blockchain efficiency (\S\ref{subsec:blockchainEff}) and security (\S\ref{subsec:sec}), and the impact mining pools have on each of these.


%The remainder of this paper is organized as follows.
%\S\ref{bg} provides essential background on permissionless blockchains in general and Ethereum in particular.
%\S\ref{methodology} describes our measurement infrastructure and methodology.
%\S\ref{Analysis} presents the main results of our study, while
%\S\ref{relwork} provides essential related work.
%\S\ref{Lessons} describes the lessons learned from our results
%and proposes lines for mitigating the major threats that our study identified.
%Lastly, \S\ref{conclusions} draws our final conclusions.

